Machine Learning based refinement strategies for polyhedral grids with applications to Virtual Element and polyhedral Discontinuous Galerkin methods

We propose two new strategies based on Machine Learning techniques to handle polyhedral grid refinement, to be possibly employed within an adaptive framework. The first one employs the k-means clustering algorithm to partition the points of the polyhedron to be refined. This strategy is a variation of the well known Centroidal Voronoi Tessellation. The second one employs Convolutional Neural Networks to classify the "shape" of an element so that "ad-hoc" refinement criteria can be defined. This strategy can be used to enhance existing refinement strategies, including the k-means strategy, at a low online computational cost. We test the proposed algorithms considering two families of finite element methods that support arbitrarily shaped polyhedral elements, namely the Virtual Element Method (VEM) and the Polygonal Discontinuous Galerkin (PolyDG) method. We demonstrate that these strategies do preserve the structure and the quality of the underlaying grids, reducing the overall computational cost and mesh complexity.

==> sections/temp.tex <==
\begin{figure}[p!]
    \centering
    \includegraphics[width = \linewidth]{images/uniform_refinement.jpg}
   \caption{In the first column, coarse grids of the domain $\Omega = (0,1)^3$: a grid of tetrahdera, a grid of cubes, a Voronoi grid, a grid with non-convex elements (obtained by agglomeration of small cubes) and a hybrid grid with cubes and prisms. Second to fourth columns: uniformly refined  grids by employing the cutting strategy orthogonal to the diameter (diameter), the Centroidal Voronoi Tesselation with 2 seeds strategy (CVT2) and the Convolutional Neural Network strategy (CNN). Each row corresponds to the same initial grid, while each column corresponds to the same refinement strategy. For visualization purposes grids have been represented after only one step of uniform refinement, while a total of three steps was actually performed.}
    \label{fig:corse grids refined}
\end{figure}

\begin{figure}[p!]
\centering
    \includegraphics[width = \linewidth]{images/quality_vertical.jpg}
\end{figure}

\begin{figure}[p!]
\vspace{-1cm}
    \centering
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_delaunay.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_delaunay.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_delaunay.jpg}

    \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_cube.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_cube.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_cube.jpg}
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_voro.jpg}
    
    
     \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_smooth_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_smooth_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_smooth_voro.jpg}
    
    \caption{Uniform case $\alpha = 5$.\\
    CVT CNN refinement times: 0.9268    7.4240   67.9038.\\
    CVT K-means refinement times: 1.4857   13.4965  144.3206.}
    \label{fig:DG unif}
\end{figure}

\begin{figure}[p!]
\vspace{-1cm}
    \centering
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_delaunay_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_delaunay_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_delaunay_alpha_2.jpg}

    \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_cube_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_cube_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_cube_alpha_2.jpg}
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_voro_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_voro_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_voro_alpha_2.jpg}
    
    
     \includegraphics[width = 0.32\linewidth]{images/DG_errors_unif_smooth_voro_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_unif_smooth_voro_alpha_2.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_unif_smooth_voro_alpha_2.jpg}
    
    \caption{Uniform case $\alpha = 2$.}
    \label{fig:DG unif}
\end{figure}


\begin{figure}[p!]
    \centering
    \includegraphics[width = \linewidth]{images/adaptive_refinement.jpg}
    \caption{Adaptively refined grids for the test case of Section 4. In the first column, fine grids of the domain $\Omega = (0,1)^3$: a grid of tetrahdera, a grid of cubes, a Voronoi grid, a grid with non-convex elements (obtained by agglomeration of small cubes) and a hybrid grid with cubes and prisms. Second to fourth columns: adaptively refined  grids by employing the cutting strategy orthogonal to the diameter (diameter), the Centroidal Voronoi Tesselation with 2 seeds strategy (CVT2) and the Convolutional Neural Network strategy (CNN). Each row corresponds to the same initial grid, while each column corresponds to the same refinement strategy. Three successively adaptive refinement steps have been performed, with a fixed fraction refinement criterion (refinement fraction $r$ set equal to 40\%).}
   \label{fig:fine grids refined}
\end{figure}

\begin{figure}[p!]
\vspace{-1cm}
    \centering
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_adapt_delaunay.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_adapt_delaunay.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_adapt_delaunay.jpg}

    \includegraphics[width = 0.32\linewidth]{images/DG_errors_adapt_cube.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_adapt_cube.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_adapt_cube.jpg}
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_adapt_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_adapt_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_adapt_voro.jpg}
    
    \includegraphics[width = 0.32\linewidth]{images/DG_errors_adapt_smooth_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/H1_errors_adapt_smooth_voro.jpg}
    \includegraphics[width = 0.32\linewidth]{images/L2_errors_adapt_smooth_voro.jpg}
    
    \caption{Adaptive case.}
    \label{fig:DG adapt}
\end{figure}

